Communication-Efficient Jaccard Similarity for High-Performance Distributed Genome Comparisons

The Jaccard similarity index is an important measure of the overlap of two sets, widely used in machine learning, computational genomics, information retrieval, and many other areas. We design and implement SimilarityAtScale, the first communication-efficient distributed algorithm for computing the Jaccard similarity among pairs of large datasets. Our algorithm provides an efficient encoding of this problem into a multiplication of sparse matrices. Both the encoding and sparse matrix product are performed in a way that minimizes data movement in terms of communication and synchronization costs. We apply our algorithm to obtain similarity among all pairs of a set of large samples of genomes. This task is a key part of modern metagenomics analysis and an evergrowing need due to the increasing availability of high-throughput DNA sequencing data. The resulting scheme is the first to enable accurate Jaccard distance derivations for massive datasets, using largescale distributed-memory systems. We package our routines in a tool, called GenomeAtScale, that combines the proposed algorithm with tools for processing input sequences. Our evaluation on real data illustrates that one can use GenomeAtScale to effectively employ tens of thousands of processors to reach new frontiers in large-scale genomic and metagenomic analysis. While GenomeAtScale can be used to foster DNA research, the more general underlying SimilarityAtScale algorithm may be used for high-performance distributed similarity computations in other data analytics application domains.

==> background.tex <==
\section{Notation and Fundamental Concepts}

We first describe background.  The most important symbols used in this work are
listed in Table~\ref{tab:symbols}.

\begin{table}[h]
\centering
%\footnotesize
\scriptsize
%\ssmall
\sf
%
%\begin{tabular}{@{}l|ll@{}}
%
\begin{tabular}{@{}ll@{}}
\toprule
%
$J, d_J$ & The Jaccard Similarity index and the Jaccard distance; $d_J = 1 - J$. \\
%
%\multirow{3}{*}{\begin{turn}{90}\shortstack{{Graph}\\{struct.}}\end{turn}}
%
%\multirow{5}{*}{\begin{turn}{90}\shortstack{{Algebraic}\\{notation}}\end{turn}}
                     $\otimes, \odot$ & Matrix-vector (MV); element-wise vector-vector (VV) product.\\
%                    & $\odot$ &Elementwise vector-vector (VV) multiplication.\\
%                    & $\mathbf{A},\mathbf{A'}$& $G$'s adjacency matrix and the transformed $\mathbf{A}$ used in~\cref{sec:tropical}.\\
%                    & $\mathbf{x}_k,\mathbf{f}_k$& The result of $\mathbf{A} \otimes \mathbf{f}_k$; the frontier of vertices in iteration~$k$.\\
%                    & $\mathbf{g}_k,\mathbf{p}_k$& Helper vectors used in boolean, real, and sel-max semirings; see~\cref{sec:accelerate_bfs_variants}.\\
%                    & $\mathbf{d}, \mathbf{p}$ & Distances (to the root) and parents (in th BFS traversal tree). \\
%                    & $DP(\mathbf{d})$ & A transformation that derives vertex parents $\mathbf{p}$ from $\mathbf{d}$. \\
%                    & $\mathbf{x}^s,\mathbf{x}_k$ &$s$th element of a vector $\mathbf{x}$ and a vector $\mathbf{x}$ in $k$th iteration, respectively.\\
%                    & $\mathbf{x}_i$ &Vector x in $i$th iteration of computation.\\
%                    & $\overline{\mathbf{x}}$ &Element-wise negation of a vector $\mathbf{x}$.\\
%                   \midrule
%\multirow{3}{*}{\begin{turn}{90}\shortstack{Various}\end{turn}}
%                    & $T,W$ &The number of threads; work complexity of a given scheme.\\
%                    & $C,n_c$ &Chunk height; the number of chunks in SlimSell or Sell-$C$-$\sigma$.\\
%                    & $\sigma$ &Sorting scope in SlimSell and Sell-$C$-$\sigma$ ($\sigma \in [1,n]$).\\
\bottomrule
\end{tabular}
\vspace{-0.5em}
\caption{The most important symbols used in the paper.}
\label{tab:symbols}
%\vspace{-0.5em}
\end{table}

\subsection{Algebraic Concepts}


\subsection{Jaccard Measures}

The \emph{Jaccard Similarity index}~\cite{levandowsky1971distance} is a
statistic used to assess the similarity of sets. It is defined as the ratio of
the set intersection cardinality and the set union cardinality:

\begin{gather}
%
J(X, Y) = \frac{|X \cap Y|}{|X \cup Y|} = \frac{|X \cap Y|}{|X| + |Y| - |X \cap Y|}
%
\end{gather}

$X$ and $Y$ are sample sets. If both $X$ and $Y$ are empty, the index is
defined as $J(X,Y) = 1$.  Now, one can use $J(X,Y)$ to define the \emph{Jaccard
distance} $d_J(X,Y) = 1 - J(X,Y)$, which assesses the \emph{dissimilarity} of
sets and which is a proper \emph{metric} (on the collection of all finite
sets).

\subsection{Distance of Genome Sequences}

A plethora of works have been dedicated to formulating and accelerating the
problem of computing distances between genome
sequences~\cite{zielezinski2017alignment}. Traditionally, these works can be
divided two categories: \emph{alignment-based} and \emph{alignment-free}
methods. Alignment-based methods use the fact that the compared sequences
\emph{are both ordered}. An established tool in this category is
BLAST~\cite{altschul1990basic}. These methods, despite being mature and
accurate, are usually slow when applied to recent large genome data sets. To
alleviate these overheads, alignment-free methods were proposed. The key
notion in alignment-free methods is to ignore the ordering of the considered
sequences. This enables incorporating a broad selection of distance metrics,
many of which are fast to compute.

\maciej{Harun, could you write sth here?}


==> formulation.tex <==
\section{Algebraic Formulation}

\maciej{How much novelty here?}


